Calibration, Entropy Rates, and Memory in Language Models

Building accurate language models that capture meaningful long-term dependencies is a core challenge in natural language processing. Towards this end, we present a calibration-based approach to measure long-term discrepancies between a generative sequence model and the true distribution, and use these discrepancies to improve the model. Empirically, we show that state-of-the-art language models, including LSTMs and Transformers, are \emph{miscalibrated}: the entropy rates of their generations drift dramatically upward over time. We then provide provable methods to mitigate this phenomenon. Furthermore, we show how this calibration-based approach can also be used to measure the amount of memory that language models use for prediction.

==> error_amplification.tex <==
\section{Error Amplification and Calibration }\label{sec:calibration}
\sk{might be better to merge this section with the entropy rate one.}

\subsection{Error amplification under our model}
Let $f:[M]^T\rightarrow \cR$ be a function on $T$ length sequences.
Let the mean and variance of $f$ under distribution $\mathcal{D}$ be
denoted by $\mu_{\mathcal{D}}(f)$ and $\sigma^2_{\mathcal{D}}(f)$, i.e.
\begin{eqnarray*}
\mu_{\mathcal{D}}(f) &:=& \E_{w_{1:T} \sim \mathcal{D}}[ f(w_{1:T})] \, .\\
\sigma^2_{\mathcal{D}}(f) &:=& \E_{w_{1:T} \sim \mathcal{D}}[ (f(w_{1:T})-\mu_{\mathcal{D}}(f))^2] \, .
\end{eqnarray*}

If $\widehat \Pr$ is an accurate model, we may hope that:
\[
\mu_{\Pr}(f) \approx \mu_{\widehat \Pr}(f)
\]
i.e. that the expected value of $f$ under the true distribution is
close to its expected value under our model.

\begin{lemma}\label{lemma:pinsker}
(Pinsker\cite{pinsker}) 
Suppose that for all $w_{1:T}$, $f(w_{1:T})\leq B$. We have that:
\[
  \left|\mu_{\Pr}(f) - \mu_{\widehat \Pr}(f)
\right|
\leq B \sqrt{\textrm{KL}(\Pr || \widehat \Pr)} \, .
\]
\end{lemma}

\subsection{Model calibration to $f$}

Define the distribution $\widehat \Pr_\alpha$ such that:
\begin{multline*}
  \widehat \Pr_\alpha(w_{1:T})  = \frac{\exp(-\alpha f(w_{1:T})) \cdot \widehat
    \Pr(w_{1:T})}{Z_\alpha}\\
  \textrm{ where } Z_\alpha
  =\sum_{w_{1:T}}\exp(-\alpha f(w_{1:T})) \cdot \widehat
  \Pr(w_{1:T})\, .
\end{multline*}

\begin{theorem}\label{thm:calibration}
(calibration and model improvement)
Suppose the variance of $f$ is uniformly bounded in that there exists
$\sigma^2_+$ such that the following holds for all
$\alpha$,
\[
\sigma^2_{\Pr_\alpha}(f)
  \leq \sigma^2_+ \, .
\]
Let
\[
\alpha^* = \argmin_{\alpha}   \mathrm{CE}(\Pr || \widehat \Pr_\alpha)\, .
\]
We have 
\[
\mu_{\Pr}(f) -  \mu_{\widehat \Pr_{\alpha^*}}(f) = 0
\]
and 
\begin{multline*}
  \mathrm{CE}(\Pr ||\widehat \Pr_{\alpha^*}) \leq \\  \mathrm{CE}(\Pr ||\widehat
  \Pr) - \frac{1}{T}\frac{( \mu(f) -  \mu_{\widehat \Pr}(f))^2}{2\sigma^2_*} \, .
\end{multline*}
\end{theorem}

\kn{need to add in implications, example of f=H + calibration algorithm}

==> experiments.tex <==
\section{Experimental Details}\label{sec:experiments}
% In this section, we outline the experimental setups used to obtain the empirical results throughout the paper.
For the calibration and memory experiments (Table~\ref{table:ent_rate_amplification} row 1, Figure~\ref{fig:entrate} (top), Figures~\ref{fig:entrate-fix},~\ref{fig:memory}), our base model is a 3-layer LSTM with with 400 embedding dimension and 1150 hidden nodes. We train it on the Penn Treebank (PTB) corpus \cite{marcus1993building}, following the setup of~\cite{merityRegOpt} and~\cite{merityAnalysis} for 500 epochs using SGD with batch size 20 and BPTT length 70. The trained base model achieves 64.3 validation perplexity and 58.3 test perplexity.

The limited-memory models $\widetilde \Pr(\cdot|W_{t-\tau:t-1})$ used for the memory estimation in section~\ref{sec:memory_estimate} share the same architecture as our base model while, during training, the hidden states is re-initialized after reading every $\tau$ tokens ($\tau$ takes value from $\{5, 15, \ldots, 30\}$).

Finally, for the other entropy rate measurements (Table~\ref{table:ent_rate_amplification} rows 2-3, Figure~\ref{fig:entrate} (bottom)), we used the pretrained weights published alongside \cite{jozefowicz2016exploring,radford2019language}. The former is an LSTM with CNN-embedded inputs, trained on the Google Billion Words (GBW) corpus. The latter is a Transformer \cite{vaswani} model trained on a corpus derived from a web crawl (WebText). For GPT-2, since the authors have not published training or validation data, we used the text of several New York Times articles as a stand-in validation set; the cross entropy loss is comparable to that reported on the validation set. %in the paper.

To measure the conditional entropy after $t$ generations, we measured the empirical conditional entropy of the $t$-th word over $>500$ independent generations, which were produced by the standard way of iteratively sampling from the next predicted conditional distribution, seeded with ground-truth text up to $>100$ random points in the validation set. We used the entropy rate at $t = 700$ as a proxy for the asymptotic limit in Table~\ref{table:ent_rate_amplification}.
